Goal-oriented Data Warehouse Quality Measurement

Requirements engineering is known to be a key factor for the success of software projects. Inside this discipline, goal-oriented requirements engineering approaches have shown specially suitable to deal with projects where it is necessary to capture the alignment between system requirements and stakeholders' needs, as is the case of data-warehousing projects. However, the mere alignment of data-warehouse system requirements with business goals is not enough to assure better data-warehousing products; measures and techniques are also needed to assure the data-warehouse quality. In this paper, we provide a modelling framework for data-warehouse quality measurement (i*DWQM). This framework, conceived as an i* extension, provides support for the definition of data-warehouse requirements analysis models that include quantifiable quality scenarios, defined in terms of well-formed measures. This extension has been defined by means of a UML profiling architecture. The resulting framework has been implemented in the Eclipse development platform.

==> pkgs.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FILENAME: Package Usage
% ----------------------------------------------------------------------------
% AUTHOR: Jesús Pardillo (jesuspv@dlsi.ua.es)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% COMMENTS:
% - The package are listed alphabetically
% - Each package is followed by its configuration and derived parameters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% graphics for LaTeX!

\usepackage{ifpdf}

\ifpdf
\usepackage[pdftex]{graphicx}
\DeclareGraphicsExtensions{.pdf,.png}
\else
\usepackage[dvips]{graphicx}
\DeclareGraphicsExtensions{.eps,.ps}
\fi

% figure location (extension don't matter)
\graphicspath{{./img/}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{multirow}
\usepackage{color}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

